Compositional Generalization via Neural-Symbolic Stack Machines

Despite achieving tremendous success, existing deep learning models have exposed limitations in compositional generalization, the capability to learn compositional rules and apply them to unseen cases in a systematic manner. To tackle this issue, we propose the Neural-Symbolic Stack Machine (NeSS). It contains a neural network to generate traces, which are then executed by a symbolic stack machine enhanced with sequence manipulation operations. NeSS combines the expressive power of neural sequence models with the recursion supported by the symbolic stack machine. Without training supervision on execution traces, NeSS achieves 100% generalization performance in four domains: the SCAN benchmark of language-driven navigation tasks, the task of few-shot learning of compositional instructions, the compositional machine translation benchmark, and context-free grammar parsing tasks.

==> architecture.tex <==
\section{Neural-Symbolic Stack Machine (\ours)}
\label{sec:approach}
In this section, we present the design of {\ours}, which includes a symbolic stack machine enhanced with sequence manipulation operations, and a neural network as the machine controller that produces a trace to be executed by the machine.
\subsection{Stack Machine Augmented with a Memory}
\label{sec:machine}

We design a stack machine augmented with a memory, a general-purpose machine for sequence-to-sequence generation that supports recursion and rule extraction, so as to achieve compositional generalization. We present an overview of the machine operations in Table~\ref{tab:stack-machine}. Specifically, \shift is used for reading the input sequence, \push and \pop are standard stack operations, \reduce is used for output sequence generation, \concatm and \concats are used to concatenate the generated sentences to form a longer one, and a \final instruction terminates the machine operation and produces the output. We provide an illustrative example in Figure~\ref{fig:stack-machine}, and defer more descriptions to the supplementary material.

\begin{table}[tbp]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{lll}
    \toprule
    \bf{Instruction} & \bf{Arguments} & \bf{Description} \\
    \midrule
    \shift & $-$ & Pull one token from the input stream to append to the end of the stack top. \\
    \midrule
    \reduce & [$t_1$, $t_2$, ..., $t_l$] & Reduce the stack's top to a sequence [$t_1$, $t_2$, ..., $t_l$] in the target language. \\
    \midrule
    \push & $-$ & Push a new frame at the stack top. \\
    \midrule
    \pop & $-$ & Pop the stack top and append the popped data to the new stack top. \\
    \midrule
    \multirow{2}{*}{\concatm} & \multirow{2}{*}{[$i_1$, $i_2$, ..., $i_l$]} & Concatenate the items from the stack top and the memory with indices $i_1$, $i_2$, ..., $i_l$, \\
    & & then put the concatenated sequence in the memory. \\
    \midrule
    \multirow{2}{*}{\concats} & \multirow{2}{*}{[$i_1$, $i_2$, ..., $i_l$]}  & Concatenate the items from the stack top and the memory with indices $i_1$, $i_2$, ..., $i_l$, \\
    & & then put the concatenated sequence in the stack.  \\
    \midrule
    \final & $-$ & Terminate the execution, and return the stack top as the output. \\
    \bottomrule
    \end{tabular}}
    \caption{Instruction semantics of the stack machine. See Figure~\ref{fig:stack-machine} for the sample usage.}
    \label{tab:stack-machine}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=1.05\linewidth]{fig/stack-machine.png}
    \caption{An illustrative example of how to use the stack machine for SCAN benchmark. A more complex example can be found in the supplementary material.}
    \label{fig:stack-machine}
\end{figure}

\subsection{The Expressive Power of {\ours}}
\label{sec:expressiveness}

In this section, we provide a detailed discussion between {\ours} and most relevant neural model architectures, including neural-symbolic approaches~\cite{chen2017towards} and sequence-to-sequence models~\cite{bahdanau2014neural,vaswani2017attention}. We will draw a connection with more existing work in Section~\ref{sec:work}.

\paragraph{Connection to neural SHIFT-REDUCE parsers.} There is a line work studying a neural network to operate a SHIFT-REDUCE system for parsing~\cite{cross2016span,misra2016neural,liu2017shift,chen2017towards}. In particular, the design of our neural-symbolic architecture is inspired by the neural parser introduced in~\cite{chen2017towards}, which was designed to produce parse trees for inputs satisfying context-free grammars. Specifically, \shift, \push, \pop and \final instructions of our machine share the same semantics as the LL machine operated by their neural parsing model, and we incorporate their stack design to support recursion. However, there are several key differences in terms of the design purpose and expressiveness. Firstly, their machine is specialized for parse tree generation, while our machine is designed for sequence generation. Therefore, although both machines support the \reduce instruction, a \reduce instruction of the LL machine generates a non-terminal and selects children from the top stack frame to construct a tree, while our machine applies a \reduce instruction to generate a sequence. Meanwhile, the memory module enables our machine to preserve some intermediate execution results, so that the same element may participate in multiple execution steps, which is essential for handling cases beyond context-free grammars. By serializing the target parse tree, our machine is capable of fully covering the usages supported by the LL machine, and we provide an illustration in the supplementary material. On the other hand, the incorporation of a memory module and enhanced instructions for sequence generation provide our machine with better expressiveness. In Section~\ref{sec:eval}, we demonstrate that {\ours} achieves $100\%$ generalization performance on the challenging context-free grammar parsing tasks in~\cite{chen2017towards}, while also provides strong results in other domains.

\paragraph{Connection to end-to-end sequence-to-sequence models.} When we pose no constraints to regularize the machine, e.g., we do not restrict the maximal number of arguments for each \reduce instruction, an execution trace that could be valid for every input-output example is to keep running \shift instruction until an $\verb|[EOS]|$ is observed as the next input token, then execute a \reduce instruction with the entire output sequence as its arguments. We call it a~\emph{degenerate} trace hereafter. In this way, the machine imitates the behavior of the sequence-to-sequence model utilized as the \reduce argument generator, which could be recurrent models~\cite{bahdanau2014neural,wiseman2016sequence,hochreiter1997long}, Transformer-based models~\cite{vaswani2017attention,devlin2018bert}, etc. To encourage the neural model to leverage the recursion property of the machine, we could set a length limit for the \reduce arguments, so that the neural model mainly calls \reduce instruction to generate phrases in the target language, and utilizes other instructions to combine the generated primitives to form a longer sequence. We call such traces with compositional behavior as~\emph{non-degenerate} traces.









==> train-old.tex <==
\section{Training Algorithm}
\label{sec:training}

To fully unlock the generalization capability of {\ours}, a main challenge is to train our {\ours} without the knowledge of the compositional rules and the ground truth execution traces that encode the alignment between the source and the target sequences. To tackle this challenge, we propose a curriculum learning scheme, which jointly learns the primitive alignment and the compositional rules, from the simplest to the most complicated ones. We outline the training algorithm in Algorithm~\ref{alg:train}, discuss the key sub-routines below, and defer more details to the supplementary material.

\begin{algorithm}[t] 
\begin{algorithmic}
\State \textbf{Input:} training lessons $L$, the $i$-th lesson $L_i=\{(x_{ij}, y_{ij})\}_{j=1}^{N_i}$, a model $p^\theta$
\State The extracted ruleset $R \leftarrow \emptyset$
\State The current training data $D \leftarrow \emptyset$
\For {$L_i \in L$}
    \State $D \leftarrow D \cup L_i$
    \Repeat
    \For {each batch $B_j=\{(x_k, y_k)\}_{k=1}^{|B_j|} \in T$}
        \State $T_j \leftarrow \text{TraceSearch}(p^\theta, B_j, R)$ // Discussed in Section~\ref{sec:search}.
        \State $I_j \leftarrow$ instruction traces in $T_j$
        \State $args_j$ = \reduce, \concatm, \concats arguments in $T_j$
        \State // $OEs$, $OEt$: latent category supervision for the source and target languages.
        \State $OEs_j, OEt_j \leftarrow \text{OEExtraction}(B_j, T_j)$ // Discussed in Section~\ref{sec:categorize}.
        \State $Loss_{\text{ins}} \leftarrow -\log p_{\text{ins}}^\theta(I_j)$, $Loss_{args} \leftarrow -\log p_{\text{args}}^\theta(args_j)$
        \State $Loss_{\text{OE}} \leftarrow -(\log p_{sc}(OEs_j) + \log p_{tc}(OEt_j)$)
        \State $Loss \leftarrow Loss_{\text{ins}} + Loss_{\text{args}} + Loss_{\text{OE}}$
        \State Update $\theta$ to minimize $Loss$
    \EndFor
    \Until{No more non-degenerate execution traces are found with the search.}
    \State $R \leftarrow \text{RuleExtraction}(p^\theta, L_i)$ // Discussed in Section~\ref{sec:search}.
\EndFor
\end{algorithmic}
\caption{Training algorithm for {\ours}}
\label{alg:train}
\end{algorithm}

\subsection{Neural-guided Trace Search with Extracted Rules}
\label{sec:search}

To obtain training supervision, for each input sequence within the current lesson, we search for an execution trace that leads to the ground truth output, based on the probability distribution predicted by the neural model, and we prioritize the search for non-degenerate execution traces. If the model could not find any non-degenerate execution trace within the search budget, a degenerate execution trace is used for training.

This search procedure works well when the input and output sequences are short. However, when the sequences grow longer, the search space of execution traces could be intractable. Therefore, during the curriculum learning process, we extract rules from previous lessons to guide the search for the current lesson, which are represented as tuples of machine statuses and their corresponding operations. For example, after learning the translation rules of ``walk'' and ``jump'', they could be utilized to translate longer sequences such as ``walk after jump''. Specifically, when the model encounters a machine status that occurs in the rule set extracted from previous lessons, the search process prioritizes the usage of the instruction and arguments specified by the corresponding rule, thus the model could leverage the knowledge acquired from previous lessons to a better extent. We discuss the details of the rule extraction process in the supplementary material. 

\subsection{Learning to Categorize with Inferred Execution Traces}
\label{sec:categorize}

As discussed in Section~\ref{sec:architecture}, component categorization is crucial for compositional generalization. In the context of parsing, a non-terminal in the parse tree provides the categorical information of the token sequence included in the sub-tree rooted at the non-terminal. Therefore, similar to the neural parser architecture proposed in~\cite{chen2017towards}, we leverage the knowledge of non-terminals provided in the ground truth parse trees as training supervision, which enables the neural model to group input tokens associated with the same non-terminal together, so that they share some common execution steps to operate the machine. However, such structural annotations are typically unavailable or expensive to obtain in the datasets. For example, on SCAN benchmarks, from pairs of input and output sequences without additional annotation, the model needs to infer that both ``walk'' and ``jump'' are primitive actions, while ``and'' and ``after'' are connectives. Without learning to compare and contrast different constituents, the model could hardly generalize when provided with a new primitive or a novel combination of seen components.

To supply such compositional inductive bias, we utilize the execution traces collected in the search process, which indicate the~\emph{operational equivalence} of two token sequences. In the following, we provide a formal definition of the operational equivalence studied in this work.

\begin{defi} [Operational Equivalence (OE).] Let $\mathcal{L}_s$, $\mathcal{L}_t$ be the source and target languages, $\pi$ be the mapping between $\mathcal{L}_s$ and $\mathcal{L}_t$; $I(s)$ be the instruction trace (i.e., the execution trace excluding the arguments) executed to perform the mapping $\pi$, where $s$ is the machine status; $\mathcal{S}$ be the set of valid machine statuses subject to $\pi$; $R(s, s_i, s'_i)$ means replacing the occurrences of $s_i$ in $s$ with $s'_i$, where $s_i$ and $s'_i$ are possible components included in the machine status. $s_i$ and $s'_i$ are operational equivalent if and only if for any machine status $s \in \mathcal{S}$, $s'=R(s, s_i, s'_i) \in \mathcal{S}$ and $I(s)=I(s')$. \adams{Shorten it?}
\end{defi}

In Figure~\ref{fig:operational-equivalence}, we present some examples of operational equivalence captured by the execution traces. We observe that when two tokens only trigger the difference in terms of the \reduce arguments, they correspond to different primitives of the same category, which is the main focus of most prior work on compositional generalization~\cite{gordon2019permutation,li2019compositional,lake2019compositional}; for example, in~\cite{gordon2019permutation}, they propose the notation of~\emph{local equivariance} to capture such equivalence. On the other hand, by grouping two token sequences only differ in the \concatm and \concats arguments, we also allow the model to capture structural equivalence, as shown in Figure~\ref{fig:global-equivariance}. This is the key to enable generalization beyond primitive substitutions, which has been a long-standing challenge. By learning latent category predictors for trace prediction, our neural controller is trained to achieve operational equivalence for sequence-to-sequence generation.

In practice, it is infeasible to enumerate all possible combinations of components to find the operationally equivalent ones. To provide training supervision for latent category predictors in an efficient way, after the search of execution traces for each input-output pair in the training batch, we collect the non-degenerate instruction traces and compare among different samples. If two samples share the same instruction trace, we mark tokens with the same indices of the input sequences, as well as their target sequences, as candidates of operationally equivalent ones, and assign the same category for training supervision. More training details of the latent category predictors are discussed in the supplementary material.

\begin{figure}
    \centering
    \begin{subfigure}[t]{\linewidth}
    \includegraphics[width=\linewidth]{fig/local-equivariance.png}
    \caption{}
    \label{fig:local-equivariance}
    \end{subfigure}
    \begin{subfigure}[t]{\linewidth}
    \includegraphics[width=\linewidth]{fig/global-equivariance.png}
    \caption{}
    \label{fig:global-equivariance}
    \end{subfigure}
    \caption{An illustration of the operational equivalence captured by the execution traces on SCAN benchmark. (a) With primitive replacement, e.g., changing ``run'' into ``jump'', the instruction trace remains the same, while the \reduce arguments differ. Such equivalence is also characterized by local equivariance defined in~\cite{gordon2019permutation}. (b) With adverb replacement, e.g., changing ``twice'' into ``thrice'', the instruction trace remains the same, while the \concatm and \concats arguments could differ. Such equivalence is crucial in achieving length generalization on SCAN, which is not characterized by primitive equivariance studied in prior work~\cite{gordon2019permutation,li2019compositional,lake2019compositional}}
    \label{fig:operational-equivalence}
\end{figure}



